A Survey on Using Gaze Behaviour for Natural Language Processing

Gaze behaviour has been used as a way to gather cognitive information for a number of years. In this paper, we discuss the use of gaze behaviour in solving different tasks in natural language processing (NLP) without having to record it at test time. This is because the collection of gaze behaviour is a costly task, both in terms of time and money. Hence, in this paper, we focus on research done to alleviate the need for recording gaze behaviour at run time. We also mention different eye tracking corpora in multiple languages, which are currently available and can be used in natural language processing. We conclude our paper by discussing applications in a domain - education - and how learning gaze behaviour can help in solving the tasks of complex word identification and automatic essay grading.

==> Instructions.tex <==
\section{Introduction}

The {\it IJCAI--20 Proceedings} will be printed from electronic manuscripts submitted by the authors. These must be PDF ({\em Portable Document Format}) files formatted for 8-1/2$''$ $\times$ 11$''$ paper.

\subsection{Length of Papers}

All paper {\em submissions} must have a maximum of six pages, plus at most one for references. The seventh page cannot contain {\bf anything} other than references.

The length rules may change for final camera-ready versions of accepted papers and will differ between tracks. Some tracks may include only references in the last page, whereas others allow for any content in all pages. Similarly, some tracks allow you to buy a few extra pages should you want to, whereas others don't.

If your paper is accepted, please carefully read the notifications you receive, and check the proceedings submission information website\footnote{\url{https://proceedings.ijcai.org/info}} to know how many pages you can finally use. That website holds the most up-to-date information regarding paper length limits at all times. Please notice that if your track allows for a special references-only page, the {\bf references-only page(s) cannot contain anything else than references} (i.e.: do not write your acknowledgments on that page or you will be charged for it).

\subsection{Word Processing Software}

As detailed below, IJCAI has prepared and made available a set of \LaTeX{} macros and a Microsoft Word template for use in formatting your paper. If you are using some other word processing software, please follow the format instructions given below and ensure that your final paper looks as much like this sample as possible.

\section{Style and Format}

\LaTeX{} and Word style files that implement these instructions can be retrieved electronically. (See Appendix~\ref{stylefiles} for instructions on how to obtain these files.)

\subsection{Layout}

Print manuscripts two columns to a page, in the manner in which these instructions are printed. The exact dimensions for pages are:
\begin{itemize}
\item left and right margins: .75$''$
\item column width: 3.375$''$
\item gap between columns: .25$''$
\item top margin---first page: 1.375$''$
\item top margin---other pages: .75$''$
\item bottom margin: 1.25$''$
\item column height---first page: 6.625$''$
\item column height---other pages: 9$''$
\end{itemize}

All measurements assume an 8-1/2$''$ $\times$ 11$''$ page size. For A4-size paper, use the given top and left margins, column width, height, and gap, and modify the bottom and right margins as necessary.

\subsection{Format of Electronic Manuscript}

For the production of the electronic manuscript, you must use Adobe's {\em Portable Document Format} (PDF). A PDF file can be generated, for instance, on Unix systems using {\tt ps2pdf} or on Windows systems using Adobe's Distiller. There is also a website with free software and conversion services: \url{http://www.ps2pdf.com}. For reasons of uniformity, use of Adobe's {\em Times Roman} font is strongly suggested. In \LaTeX2e{} this is accomplished by writing
\begin{quote} 
\mbox{\tt $\backslash$usepackage\{times\}}
\end{quote}
in the preamble.\footnote{You may want also to use the package {\tt latexsym}, which defines all symbols known from the old \LaTeX{} version.}

Additionally, it is of utmost importance to specify the {\bf letter} format (corresponding to 8-1/2$''$ $\times$ 11$''$) when formatting the paper. When working with {\tt dvips}, for instance, one should specify {\tt -t letter}.

\subsection{Title and Author Information}

Center the title on the entire width of the page in a 14-point bold font. The title must be capitalized using Title Case. Below it, center author name(s) in 12-point bold font. On the following line(s) place the affiliations, each affiliation on its own line using 12-point regular font. Matching between authors and affiliations can be done using numeric superindices. Optionally, a comma-separated list of email addresses follows the affiliation(s) line(s), using 12-point regular font.

\subsubsection{Blind Review}

In order to make blind reviewing possible, authors must omit their names and affiliations when submitting the paper for review. In place of names and affiliations, provide a list of content areas. When referring to one's own work, use the third person rather than the first person. For example, say, ``Previously, Gottlob~\shortcite{gottlob:nonmon} has shown that\ldots'', rather than, ``In our previous work~\cite{gottlob:nonmon}, we have shown that\ldots'' Try to avoid including any information in the body of the paper or references that would identify the authors or their institutions. Such information can be added to the final camera-ready version for publication.

\subsection{Abstract}

Place the abstract at the beginning of the first column 3$''$ from the top of the page, unless that does not leave enough room for the title and author information. Use a slightly smaller width than in the body of the paper. Head the abstract with ``Abstract'' centered above the body of the abstract in a 12-point bold font. The body of the abstract should be in the same font as the body of the paper.

The abstract should be a concise, one-paragraph summary describing the general thesis and conclusion of your paper. A reader should be able to learn the purpose of the paper and the reason for its importance from the abstract. The abstract should be no more than 200 words long.

\subsection{Text}

The main body of the text immediately follows the abstract. Use 10-point type in a clear, readable font with 1-point leading (10 on 11).

Indent when starting a new paragraph, except after major headings.

\subsection{Headings and Sections}

When necessary, headings should be used to separate major sections of your paper. (These instructions use many headings to demonstrate their appearance; your paper should have fewer headings.). All headings should be capitalized using Title Case.

\subsubsection{Section Headings}

Print section headings in 12-point bold type in the style shown in these instructions. Leave a blank space of approximately 10 points above and 4 points below section headings. Number sections with arabic numerals.

\subsubsection{Subsection Headings}

Print subsection headings in 11-point bold type. Leave a blank space of approximately 8 points above and 3 points below subsection headings. Number subsections with the section number and the subsection number (in arabic numerals) separated by a period.

\subsubsection{Subsubsection Headings}

Print subsubsection headings in 10-point bold type. Leave a blank space of approximately 6 points above subsubsection headings. Do not number subsubsections.

\paragraph{Titled paragraphs.} You should use titled paragraphs if and only if the title covers exactly one paragraph. Such paragraphs should be separated from the preceding content by at least 3pt, and no more than 6pt. The title should be in 10pt bold font and ended with a period. After that, a 1em horizontal space should follow the title before the paragraph's text.

In \LaTeX{} titled paragraphs should be typeset using
\begin{quote}
{\tt \textbackslash{}paragraph\{Title.\} text} .
\end{quote}

\subsubsection{Acknowledgements}

You may include an unnumbered acknowledgments section, including acknowledgments of help from colleagues, financial support, and permission to publish. If present, acknowledgements must be in a dedicated, unnumbered section appearing after all regular sections but before any appendices or references.

Use 
\begin{quote}
    {\tt \textbackslash{}section*\{Acknowledgements\}})
\end{quote}
to typeset the acknowledgements section in \LaTeX{}.

\subsubsection{Appendices}

Any appendices directly follow the text and look like sections, except that they are numbered with capital letters instead of arabic numerals. See this document for an example.

\subsubsection{References}

The references section is headed ``References'', printed in the same style as a section heading but without a number. A sample list of references is given at the end of these instructions. Use a consistent format for references. The reference list should not include unpublished work.

\subsection{Citations}

Citations within the text should include the author's last name and the year of publication, for example~\cite{gottlob:nonmon}.  Append lowercase letters to the year in cases of ambiguity.  Treat multiple authors as in the following examples:~\cite{abelson-et-al:scheme} or~\cite{bgf:Lixto} (for more than two authors) and \cite{brachman-schmolze:kl-one} (for two authors). If the author portion of a citation is obvious, omit it, e.g., Nebel~\shortcite{nebel:jair-2000}.  Collapse multiple citations as follows:~\cite{gls:hypertrees,levesque:functional-foundations}.

\subsection{Footnotes}

Place footnotes at the bottom of the page in a 9-point font. Refer to them with superscript numbers.\footnote{This is how your footnotes should appear.} Separate them from the text by a short line.\footnote{Note the line separating these footnotes from the text.} Avoid footnotes as much as possible; they interrupt the flow of the text.

\section{Illustrations}

Place all illustrations (figures, drawings, tables, and photographs) throughout the paper at the places where they are first discussed, rather than at the end of the paper.

They should be floated to the top (preferred) or bottom of the page, unless they are an integral part of your narrative flow. When placed at the bottom or top of a page, illustrations may run across both columns, but not when they appear inline.

Illustrations must be rendered electronically or scanned and placed directly in your document. They should be cropped outside latex, otherwise portions of the image could reappear during the post-processing of your paper. All illustrations should be understandable when printed in black and white, albeit you can use colors to enhance them. Line weights should be 1/2-point or thicker. Avoid screens and superimposing type on patterns, as these effects may not reproduce well.

Number illustrations sequentially. Use references of the following form: Figure 1, Table 2, etc. Place illustration numbers and captions under illustrations. Leave a margin of 1/4-inch around the area covered by the illustration and caption.  Use 9-point type for captions, labels, and other text in illustrations. Captions should always appear below the illustration.

\section{Tables}

Tables are considered illustrations containing data. Therefore, they should also appear floated to the top (preferably) or bottom of the page, and with the captions below them.

\begin{table}
\centering
\begin{tabular}{lll}
\hline
Scenario  & $\delta$ & Runtime \\
\hline
Paris       & 0.1s  & 13.65ms     \\
Paris       & 0.2s  & 0.01ms      \\
New York    & 0.1s  & 92.50ms     \\
Singapore   & 0.1s  & 33.33ms     \\
Singapore   & 0.2s  & 23.01ms     \\
\hline
\end{tabular}
\caption{Latex default table}
\label{tab:plain}
\end{table}

\begin{table}
\centering
\begin{tabular}{lrr}  
\toprule
Scenario  & $\delta$ (s) & Runtime (ms) \\
\midrule
Paris       & 0.1  & 13.65      \\
            & 0.2  & 0.01       \\
New York    & 0.1  & 92.50      \\
Singapore   & 0.1  & 33.33      \\
            & 0.2  & 23.01      \\
\bottomrule
\end{tabular}
\caption{Booktabs table}
\label{tab:booktabs}
\end{table}

If you are using \LaTeX, you should use the {\tt booktabs} package, because it produces better tables than the standard ones. Compare Tables \ref{tab:plain} and \ref{tab:booktabs}. The latter is clearly more readable for three reasons:

\begin{enumerate}
\item The styling is better thanks to using the {\tt booktabs} rulers instead of the default ones.
\item Numeric columns are right-aligned, making it easier to compare the numbers. Make sure to also right-align the corresponding headers, and to use the same precision for all numbers.
\item We avoid unnecessary repetition, both between lines (no need to repeat the scenario name in this case) as well as in the content (units can be shown in the column header).
\end{enumerate}

\section{Formulas}

IJCAI's two-column format makes it difficult to typeset long formulas. A usual temptation is to reduce the size of the formula by using the {\tt small} or {\tt tiny} sizes. This doesn't work correctly with the current \LaTeX{} versions, breaking the line spacing of the preceding paragraphs and title, as well as the equation number sizes. The following equation demonstrates the effects (notice that this entire paragraph looks badly formatted):
%
\begin{tiny}
\begin{equation}
    x = \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i
\end{equation}
\end{tiny}%

Reducing formula sizes this way is strictly forbidden. We {\bf strongly} recommend authors to split formulas in multiple lines when they don't fit in a single line. This is the easiest approach to typeset those formulas and provides the most readable output%
%
\begin{align}
    x =& \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \nonumber\\
    + & \prod_{i=1}^n \sum_{j=1}^n j_i
\end{align}%

If a line is just slightly longer than the column width, you may use the {\tt resizebox} environment on that equation. The result looks better and doesn't interfere with the paragraph's line spacing: %
\begin{equation}
\resizebox{.91\linewidth}{!}{$
    \displaystyle
    x = \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i
$}
\end{equation}%

This last solution may have to be adapted if you use different equation environments, but it can generally be made to work. Please notice that in any case:

\begin{itemize}
\item Equation numbers must be in the same font and size than the main text (10pt).
\item Your formula's main symbols should not be smaller than {\small small} text (9pt).
\end{itemize}

For instance, the formula
%
\begin{equation}
    \resizebox{.91\linewidth}{!}{$
    \displaystyle
    x = \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j + \prod_{i=1}^n \sum_{j=1}^n j_i + \prod_{i=1}^n \sum_{j=1}^n i_j
$}
\end{equation}
% 
would not be acceptable because the text is too small.

\section{Examples, Definitions, Theorems and Similar}

Examples, definitions, theorems, corollaries and similar must be written in their own paragraph. The paragraph must be separated by at least 2pt and no more than 5pt from the preceding and succeeding paragraphs. They must begin with the kind of item written in 10pt bold font followed by their number (e.g.: Theorem 1), optionally followed by a title/summary between parentheses in non-bold font and ended with a period. After that the main body of the item follows, written in 10 pt italics font (see below for examples). 

In \LaTeX{} We strongly recommend you to define environments for your examples, definitions, propositions, lemmas, corollaries and similar. This can be done in your \LaTeX{} preamble using \texttt{\textbackslash{newtheorem}} -- see the source of this document for examples. Numbering for these items must be global, not per-section (e.g.: Theorem 1 instead of Theorem 6.1).

\begin{example}[How to write an example]
Examples should be written using the example environment defined in this template.
\end{example}

\begin{theorem}
This is an example of an untitled theorem.
\end{theorem}

You may also include a title or description using these environments as shown in the following theorem.

\begin{theorem}[A titled theorem]
This is an example of a titled theorem.
\end{theorem}

\section{Proofs}

Proofs must be written in their own paragraph separated by at least 2pt and no more than 5pt from the preceding and succeeding paragraphs. Proof paragraphs should start with the keyword ``Proof." in 10pt italics font. After that the proof follows in regular 10pt font. At the end of the proof, an unfilled square symbol (qed) marks the end of the proof.

In \LaTeX{} proofs should be typeset using the \texttt{\textbackslash{proof}} environment.

\begin{proof}
This paragraph is an example of how a proof looks like using the \texttt{\textbackslash{proof}} environment. 
\end{proof}

\section{Algorithms and Listings}

Algorithms and listings are a special kind of figures. Like all illustrations, they should appear floated to the top (preferably) or bottom of the page. However, their caption should appear in the header, left-justified and enclosed between horizontal lines, as shown in Algorithm~\ref{alg:algorithm}. The algorithm body should be terminated with another horizontal line. It is up to the authors to decide whether to show line numbers or not, how to format comments, etc.

In \LaTeX{} algorithms may be typeset using the {\tt algorithm} and {\tt algorithmic} packages, but you can also use one of the many other packages for the task.  

\begin{algorithm}[tb]
\caption{Example algorithm}
\label{alg:algorithm}
\textbf{Input}: Your algorithm's input\\
\textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: Your algorithm's output
\begin{algorithmic}[1] %[1] enables line numbers
\STATE Let $t=0$.
\WHILE{condition}
\STATE Do some action.
\IF {conditional}
\STATE Perform task A.
\ELSE
\STATE Perform task B.
\ENDIF
\ENDWHILE
\STATE \textbf{return} solution
\end{algorithmic}
\end{algorithm}

\section*{Acknowledgments}

The preparation of these instructions and the \LaTeX{} and Bib\TeX{} files that implement them was supported by Schlumberger Palo Alto Research, AT\&T Bell Laboratories, and Morgan Kaufmann Publishers. Preparation of the Microsoft Word file was supported by IJCAI.  An early version of this document was created by Shirley Jowell and Peter F. Patel-Schneider. It was subsequently modified by Jennifer Ballentine and Thomas Dean, Bernhard Nebel, Daniel Pagenstecher, Kurt Steinkraus, Toby Walsh and Carles Sierra. The current version has been prepared by Marc Pujol-Gonzalez and Francisco Cruz-Mencia.

\appendix

\section{\LaTeX{} and Word Style Files}\label{stylefiles}

The \LaTeX{} and Word style files are available on the IJCAI--PRICAI--20 website, \url{https://www.ijcai20.org/}. These style files implement the formatting instructions in this document.

The \LaTeX{} files are {\tt ijcai20.sty} and {\tt ijcai20.tex}, and the Bib\TeX{} files are {\tt named.bst} and {\tt ijcai20.bib}. The \LaTeX{} style file is for version 2e of \LaTeX{}, and the Bib\TeX{} style file is for version 0.99c of Bib\TeX{} ({\em not} version 0.98i). The {\tt ijcai20.sty} style differs from the {\tt ijcai19.sty} file used for IJCAI--19.

The Microsoft Word style file consists of a single file, {\tt ijcai20.doc}. This template differs from the one used for IJCAI--19.

These Microsoft Word and \LaTeX{} files contain the source of the present document and may serve as a formatting sample.  

Further information on using these styles for the preparation of papers for IJCAI--PRICAI--20 can be obtained by contacting {\tt pcchair@ijcai20.org}.

==> Rough.tex <==
\section{Rough Work Here}

\subsection{Section \ref{Tasks Section} References}

\textbf{Important references that should go in this section:}

\begin{enumerate}
\item Abhijit Mishra, Michael Carl and Pushpak Bhattacharyya, A Heuristic Based Approach for Systematic Error Correction of Gaze Data for Reading, First Workshop on Eye Tracking and NLP, part of COLING 2012, Mumbai, India, 15 Dec, 2012
\end{enumerate}

\subsection{Section \ref{Gaze Behaviour Learning Section} References}

\textbf{Important references that should go here:}

\begin{enumerate}
\item Y. Long, R. Xiang, Q. Lu, CR Huang, and M. Li. (2019). Improving attention model based on cognition grounded data for sentiment analysis. IEEE Transactions on Affective Computing. - \cite{long2019improving}
\item Abhinav Deep Singh, Poojan Mehta, Samar Husain and Rajkumar Rajakrishnan (2016). Quantifying sentence complexity based on eye-tracking measures. In: Proceedings of the workshop on computational linguistics for linguistic complexity (cl4lc), pp. 202–212. - \cite{singh-etal-2016-quantifying}
\end{enumerate}

\begin{table}[b]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Paper} & \textbf{NLP Tasks} & \textbf{Model} & \textbf{Results} \\ \hline
\cite{klerke-etal-2016-improving} & \checkmark & \checkmark & \checkmark \\
\cite{barrett-etal-2016-pos-tagging} & \checkmark & \checkmark & \checkmark \\
\cite{gonzalez-garduno-sogaard-2017-gaze-readability} & \checkmark & \checkmark & \checkmark \\
\cite{mishra2018cognition} & \checkmark & \checkmark & \checkmark \\
\cite{hollenstein-zhang-2019-entity} & \checkmark & \checkmark & \checkmark \\
 &  &  &  \\ \hline
\end{tabular}
}%
\caption{Paper checklist}
\label{Paper checklist}
\end{table}
